Multi-particle reconstruction in the High Granularity Calorimeter using object condensation and graph neural networks

The high-luminosity upgrade of the LHC will come with unprecedented physics and computing challenges. One of these challenges is the accurate reconstruction of particles in events with up to 200 simultaneous proton-proton interactions. The planned CMS High Granularity Calorimeter offers fine spatial resolution for this purpose, with more than 6 million channels, but also poses unique challenges to reconstruction algorithms aiming to reconstruct individual particle showers. In this contribution, we propose an end-to-end machine-learning method that performs clustering, classification, and energy and position regression in one step while staying within memory and computational constraints. We employ GravNet, a graph neural network, and an object condensation loss function to achieve this task. Additionally, we propose a method to relate truth showers to reconstructed showers by maximising the energy weighted intersection over union using maximal weight matching. Our results show the efficiency of our method and highlight a promising research direction to be investigated further.

==> second.tex <==
The high-luminosity upgrade of the LHC (HL-LHC) will pose unprecedented computational challenges. In order to reach the target luminosity, collisions at the HL-LHC are planned to have an average of 200 proton-proton interactions per bunch crossing, referred to as pileup. 
Building tracks and energy clusters and associating them to their initiating pileup or primary particles in such a complex environment is a highly challenging task and requires the full event to be reconstructed in the most granular way before a decision can be made. To tackle the problem in the particularly particle-dense forward region, the calorimeter endcaps of the CMS detector will be replaced for the HL-LHC operations with the CMS High Granularity Calorimeter (HGCal), providing both fine lateral but and longitudinal segmentation. 

%here something about physics: MET PF VBS/VBF
%then this stuff:
%  e
% Out of place:
The huge combinatorics of building tracks or clusters from many neighboring hits in the detector make algorithmic approaches currently employed at the LHC infeasible. 
%and then we can connect it here, or put the ML things.

Local reconstruction of particle tracks and clusters in the HGCAL is agnostic to the full event record from the CMS detector. In particular, without the association of calorimeter tracks and clusters to the tracking detector, assigning an object to the initiating vertex, and thus to the primary interaction or to pileup, is not practical at this stage. It is therefore crucial to be able to identify and determine the properties of each individual shower down to low energy, even in case of severe overlaps with other incident particles. This makes a classic binary or sequential approach, in which an attempt it made to first separate showers and then determine their properties, suboptimal by construction. Furthermore, the individual steps, usually comprising at least one seeding step, and subsequent refinement of the object associated to the seed, all have similar pattern recognition requirements, which leads to a built-in redundancy and suboptimal usage of the computing resources.

An alternative to such a sequential reconstruction are machine-learning (ML) approaches based on the raw hit information, providing the possibility to reconstruct showers in parallel, and naturally accounting for overlapping energy deposits. Furthermore, ML algorithms are highly parallelisable and therefore exhibit a significant gain in execution speed on dedicated hardware such as graphics processing units (GPUs) or field programmable gate arrays [here we can cite a bunch of HLS4ML papers]. In particular, recent developments on graph neural networks (GNNs)~\cite{qasim2019learning} have shown promising physics potential while keeping the computing resource requirements within expected financial and technological constraints~\cite{Aarrestad:2020ngo}.
%(could we site a CMS report about computing constraints at HL-LHC as well?) Yes, we should put more here. 
These GNNs also allow abstracting from the detector geometry, which in general and in case of the HGCal is irregular.

Reconstructing multiple particles without employing seeds is a challenging problem, in particular for ML algorithms aiming to also retain the information of nearby showers until the final properties are determined. However, this issue was recently solved by object condensation~\cite{kieseler2020object}, which allows reconstructing multiple objects and their properties from irregular data in a one-shot approach by providing a method to quantify reconstruction efficiencies, noise suppression, and object property determination in a unified loss function.

Such, ML algorithms, being differentiable, can be automatically optimised for multi-particle reconstruction providing not only advantages with respect to their physics performance and execution speed due to their parallelisability, but also in terms of person power needed to fully optimise and tune the algorithm.
%[ok this paragraph can be rephrased and should go somewhere more in the beginning, but I think making this point is super important.]

This paper describes an approach  





The rest of the paper is structured as follows: Section~\ref{sec-dat} describes how the data is produced and show the distribution of it's properties. Section~\ref{sec-meth} describes the methodology, including the network, the loss function and how inference is done. In Section~\ref{sec-analy}, we propose a method to match the predictions to ground truth and then we study different performance metrics. And finally, conclusions are presented in Section~\ref{sec-conc}.
